Regularized and Opposite spin-scaled functionals from M{\o}ller-Plesset adiabatic connection -- higher accuracy at lower cost

Non-covalent interactions (NCIs) play a crucial role in biology, chemistry, material science, and everything in between. To improve pure quantum-chemical simulations of NCIs, we propose a methodology for constructing approximate correlation energies by combining an interpolation along the M{\o}ller adiabatic connection (MP AC) with a regularization and spin-scaling strategy applied to MP2 correlation energies. This combination yields $c_{\rm os}\kappa_{\rm os}$-SPL2, which exhibits superior accuracy for NCIs compared to any of the individual strategies. With the $N^4$ formal scaling, $c_{\rm os}\kappa_{\rm os}$-SPL2, is competitive or often outperforms more expensive dispersion-corrected double hybrids for NCIs.The accuracy of $c_{\rm os}\kappa_{\rm os}$-SPL2 particularly shines for anionic halogen bonded complexes, where it surpasses standard dispersion-corrected DFT by a factor of 3 to 5.

==> oldsection.tex <==
After outlining the basics of MP AC, we will briefly focus on MP2 modifications that we will use within our MP AC framework. The SCS-MP2 scheme gives the correlation energy as \cite{Gri-JCP-03}
\begin{equation}\label{eq:SCSEc}
    E_{c}^{\rm SCS-MP2}=c_{\rm os}E^{\rm MP2(OS)}_c + c_{\rm ss}E^{\rm MP2(SS)}_c,
\end{equation}
where the opposite-spin (os) and the same-spin (ss) parts are given by (closed-shell systems are assumed throughout this work):
\begin{equation}
\label{eq:OS}
    E_c^{\rm MP2(OS)} = -\sum_{abrs} \frac{\langle ab|rs\rangle^2}{\Delta_{ab}^{rs}},
\end{equation}
and
\begin{equation}\label{eq:SS}
      E_c^{\rm MP2(SS)} = -\sum_{abrs} \frac{\langle ab|rs\rangle[\langle ab|rs\rangle-\langle rs|ba\rangle]}{\Delta_{ab}^{rs}}
\end{equation}
with $\Delta_{ab}^{rs} = \epsilon_r + \epsilon_s - \epsilon_a -\epsilon_b$ being an orbital gap between a pair of occupied ($r$ and $s$) and a pair of virtual orbitals ($a$ and $b$).
The os part formally scales as $N^4$ whereas the ss part as $N^5$.  
Applying different positive scaling factors  $c_{\rm ss}, c_{\rm os}$ in Eq.~\eqref{eq:SCSEc} defines the SCS-MP2 method, while setting $c_{\rm ss}=0$ defines the cheaper scaled opposite-spin-only variant (with, e.g., $c_{\rm os}=1.4$). A more sophisticated way to improve MP2, other than the simple scaling of Eq.~\eqref{eq:SCSEc}, is to prevent divergences that appear in Eqs.~\eqref{eq:OS} and~\eqref{eq:SS}
when $\Delta_{ab}^{rs} \to 0$ through regularisation.
For example, $\kappa$-MP2 regularizes the MP2 correlation energy through $\langle{ab}||{rs}\rangle \to \langle{ab}||{rs}\rangle(1-e ^{-\kappa\Delta_{ab}^{rs}})$, resulting in the following $\kappa$-MP2 correlation energy~\cite{SheLoiRetLeeHea-JPCL-21,RetSheLeeHea-JCTC-22}
\begin{equation}\label{Ecor}
    E_{c}^{\kappa-\text{MP2}}= -\frac{1}{4} \sum_{abrs} \frac{|\langle{ab}||{rs}\rangle|^2} {\Delta_{ab}^{rs}} (1-e ^{-\kappa\Delta_{ab}^{rs}})^2.
\end{equation}
In $\kappa$-MP2$, \kappa$ is an empirical parameter, and when $\kappa=0$, 
$\kappa$-MP2 reduces to HF, whereas when $\kappa \to \infty$,  $\kappa$-MP2 reduces to 
``bare'' MP2. 
For NCI, $\kappa$-MP2 provides significant improvements over MP2, 
particularly for values $\kappa \sim 1.2$. \cite{SheLoiRetLeeHea-JPCL-21,RetSheLeeHea-JCTC-22,SanMar-JPCL-22}

\begin{table}[t]
\caption{The 6 functionals that we have studied in this work and the parameters that were fitted to the S22 dataset. 
The other 14 combinations can be found in Table S1 in the SI.}
\begin{tabular}{l||rrrrr}
   Methods        & $c_{ss}$ & $c_{os}$ &  $\kappa_{\rm ss}$ & $\kappa_{\rm os}$   \\ \hline\hline
                                                 
MP2                                   & 1 & 1& $\infty$ & $\infty$ \\
$\kappa_{\rm ss},\kappa_{\rm os}$-MP2 &  1 & 1 & 0.9 & 1.4 \\
SPL2                                  &  1 & 1 &  $\infty$ & $\infty$  \\
$\kappa_{\rm ss},\kappa_{\rm os}$-SPL2 & 1& 1 &  1.1 & 1.7 \\
$\kappa$-F1                            & 1 &1 & 1.5 & 1.5 \\
\hline
$c_{\rm os}\kappa_{\rm os}$-MP2   & 0 & 2.1 &  0 & 0.9  \\
$c_{\rm os}\kappa_{\rm os}$-SPL2   & 0 & 2.1 & 0 & 1.3  \\
$c_{\rm os}$-SPL2                  & 0 & 1.8 & $\infty$ & $\infty$ \\   
\end{tabular}
\label{tab:funcs}
%fix_below
%say where are the corresponding alpha and beta params in SI
%is it "F1" or "F1[alpha,beta]"?
\end{table}


%\begin{table}[t]
%\caption{The 6 functionals that we have studied in this work and the parameters that were %fitted to the S22 dataset. 
%The other 14 combinations can be found in Table S1 in the SI.}
%\begin{tabular}{l||l}
%   Methods        & fitted parameters \\ \hline\hline
%MP2         & $c_{\rm ss}=c_{\rm os}=1$, $\kappa_{\rm ss}=\kappa_{\rm os}=\infty$\\
%$\kappa_{\rm ss},\kappa_{\rm os}$-MP2 & $c_{\rm ss}=c_{\rm os}=1$, $\kappa_{\rm ss}=0.9$, %$\kappa_{\rm os}=1.4$\\
%SPL2        & $c_{\rm ss}=c_{\rm os}=1$, $\kappa_{\rm ss}=\kappa_{\rm os}=\infty$\\
%$\kappa_{\rm ss},\kappa_{\rm os}$-SPL2 & $c_{\rm ss}=c_{\rm os}=1$, $\kappa_{\rm ss}=1.1$, %$\kappa_{\rm os}=1.7$\\
%$\kappa$-F1 & $c_{\rm ss}=c_{\rm os}=1$, $\kappa_{\rm ss}=\kappa_{\rm os}=1.5$ \\\hline
%$c_{\rm os}\kappa_{\rm os}$-MP2   &   $c_{\rm ss}=0,c_{\rm os}=2.1$, $\kappa_{\rm %ss}=0,\kappa_{\rm os}=0.9$  \\
%$c_{\rm os}\kappa_{\rm os}$-SPL2     &   $c_{\rm ss}=0,c_{\rm os}=2.1$, $\kappa_{\rm %ss}=0,\kappa_{\rm os}=1.3$ \\
%$c_{\rm os}$-SPL2 & $c_{\rm ss}=0,c_{\rm os}=1.8$, $\kappa_{\rm ss}=\kappa_{\rm os}=\infty$   
%\end{tabular}
%\label{tab:funcs}
%%fix_below
%%say where are the corresponding alpha and beta params in SI
%%is it "F1" or "F1[alpha,beta]"?
%\end{table}

We can also combine spin-scaling and $\kappa$-regularization to MP2 to obtain:
\begin{equation}
    E_{c}^{\kappa_{\rm ss},\kappa_{\rm os}-\text{MP2}}=c_{\rm os}E_{c}^{\kappa_{\rm os}-\text{MP2}} + c_{\rm ss}E_{c}^{\kappa_{\rm ss}-\text{MP2}},
\label{eq:mp24p}
\end{equation}
with 
\begin{equation}
    E_{c}^{\kappa_{\rm os}-\text{MP2}}=-\sum_{abrs} \frac{\langle ab|rs\rangle^2}{\Delta_{ab}^{rs}}(1-e ^{-\kappa_{\rm os}\Delta_{ab}^{rs}})
\end{equation}
and
\begin{equation}
    E_{c}^{\kappa_{\rm ss}-\text{MP2}}=-\sum_{abrs} \frac{\langle ab|rs\rangle[\langle ab|rs\rangle-\langle rs|ba\rangle]}{\Delta_{ab}^{rs}}(1-e ^{-\kappa_{\rm ss}\Delta_{ab}^{rs}}). 
\end{equation}
Since in Eq.~\eqref{eq:mp24p}, $c_{\rm ss}$ and $k_{\rm ss}$
are different from their os counterparts, we have four parameters in this equation that can be fitted.
\fds{In this work, however, we consider only regularization with $c_{ss}=c_{os}=1$, thus keeping only two parameters 
($\kappa_{\rm ss},\kappa_{\rm os}$)}.
